SOTER: A Runtime Assurance Framework for Programming Safe Robotics Systems

The recent drive towards achieving greater autonomy and intelligence in robotics has led to high levels of complexity. Autonomous robots increasingly depend on third party off-the-shelf components and complex machine-learning techniques. This trend makes it challenging to provide strong design-time certification of correct operation. To address these challenges, we present SOTER, a robotics programming framework with two key components: (1) a programming language for implementing and testing high-level reactive robotics software and (2) an integrated runtime assurance (RTA) system that helps enable the use of uncertified components, while still providing safety guarantees. SOTER provides language primitives to declaratively construct a RTA module consisting of an advanced, high-performance controller (uncertified), a safe, lower-performance controller (certified), and the desired safety specification. The framework provides a formal guarantee that a well-formed RTA module always satisfies the safety specification, without completely sacrificing performance by using higher performance uncertified components whenever safe. SOTER allows the complex robotics software stack to be constructed as a composition of RTA modules, where each uncertified component is protected using a RTA module. To demonstrate the efficacy of our framework, we consider a real-world case-study of building a safe drone surveillance system. Our experiments both in simulation and on actual drones show that the SOTER-enabled RTA ensures the safety of the system, including when untrusted third-party components have bugs or deviate from the desired behavior.

==> battery_results.tex <==
\subsection{Complex safety specifications}
We implemented the above \rta module described in \shromona{insert section reference} for battery safety when the quadcopter has to travel to multiple goal locations in a given known environment. The results are shown in~\cref{Fig:battery}
\begin{wrapfigure}{l}{0.5\columnwidth}
\centering
\includegraphics[scale=0.3]{figures/battery}
\caption{Navigation with safety constraints on battery}
\label{Fig:battery}
\end{wrapfigure}
In~\cref{Fig:battery}, the grey rectangles, green circles and yellow square represents obstacles, goal locations and battery charging point respectively.

The \DM monitors the battery level and planned trajectories of the quadcopter; and when it notices the quadcopter does not have sufficient battery to cover the trajectory hands control to $\msc$. The $\msc$ then plans and executes the quickest trajectory to the battery charging station. Once the battery is charged sufficiently ($> 90\%$), the \DM hands control back to the $\mac$ and it can continue to execute the tasks.

==> batterysafety.tex <==

\subsection{Battery Safety}

\label{sec:batteryexample}
In this section, we describe how we can use our \rta module for complex safety specifications coupling the robot high-level mission and its battery level. 
A robot can safely navigate in the real world, provided it has sufficient battery. 
Battery charge is often not explicitly considered while designing a motion planner that optimizes for completing a specific task. 
Optimizing with  battery cost makes the problem harder. Hence, it would be beneficial to decouple these problems and take a more modular approach.

We would like our motion planner to provide battery-safety guarantee, that prioritizes charging the battery when it reaches below a threshold level.
To this effect, we use \rta based modular approach where the motion planner is optimized for the underlying task, while the \rta module guarantees battery-safety.

Let $T$ be the maximum battery charge required to go from any point in $\worksp$ to the battery charging point
and $b_t$ be the current battery charge. We augment the state space of the drone with $b_t$
The components of \rta are:
$\mac$ can be any motion planner; $\msc$ is designed as a safe motion planner that takes the robot from its current position to the charging point; $\phisafe$ asserts that $\bat_t > T$; $\phisafer$ asserts that $\bat_t > 95\%$.
We can define, $\ttf$ as:
$ \ttf(\bat_t) = \min_t s.t.\ \reach(b_t, *, t) \notin \phisafe$.
The resultant \rta module is well formed and satisfies battery safety properties.

Note that by wrapping the motion planner inside an \rta module that guarantees battery safety, the entire software stack satisfies the battery safety property irrespective of the application or motion planner used. The video corresponding to this experiment is available at~\url{https://drona-org.github.io/Drona/}


==> casestudy.tex <==

\section{Case Study: Autonomous Mobile Robotics System}

Our canonical application domain for the \tool runtime assurance framework is safe autonomous mobile robotics systems.
%In this paper, we motivate the need for the \tool runtime assurance framework by demonstrating its capabilities for building a safe autonomous mobile robotics system. 
In this section, we provide an overview of the robotics software stack implemented using \tool and present the terminologies, definitions needed for the rest of the paper.

\subsection{Terminology and Definitions}

%In this section, we formalize the definitions needed for the rest of the paper.

\noindent
\textbf{\textit{Workspace:}}
We represent the workspace for a robot $\worksp \subseteq \reals^3$ as a 3-D occupancy map with obstacles (Figure~\ref{fig:tubeexp}).
%The set of all locations occupied by obstacles is denoted by $\Omega$. The set of free locations in the workspace is denoted by $\floc$, where $\floc = \worksp \setminus \Omega$.

%\noindent
%\textbf{\textit{Tasks:}}
%%In an autonomous robotics system, tasks can be generated dynamically and assigned to the robot. 
%An atomic task is represented by the goal location $g \in \floc$ that the robot must visit in order to accomplish the task.
%A complex task can be represented as a sequence of atomic tasks. For example, moving from one surveillance point to another is an atomic task and periodically visiting all the surveillance points is an example of a complex task.

\noindent
\textbf{\textit{Motion primitives:}}
Motion primitives are a set of short closed-loop trajectories of a robot under the action of a set of precomputed control laws~\cite{planning_book,MellingerK11}.
The set of motion primitives form the basis of the motion of a robot. 
The low-level controllers can be used to move the robot from one location to another by continuously changing thrust.
Let $\controls$ be the set of low-level controls (e.g. torque) that can be applied to the robot.
For example, we leverage these low-level controllers to implement a motion primitive, $\goto$, that moves the robot from its current location to the goal location along a straight line joining the locations.
%We denote by $\Gamma$ the set of all motion primitives available for the robot.
%We assume that the robot is a continuous dynamical system satisfying Equation~\ref{eqn:sys}. 
We use $\pose_t$ to represent $\pose(t)$, the current location of the robot.
The $\goto$ motion primitive takes as input the destination position, $\pose_{f}$, and generates a sequence of low level controls, $u \in \controls$, to take the robot from $\pose_{t}$ to $\pose_{f}$.

\noindent
\textbf{\textit{Trajectory:}}
The trajectory $\xi$ of a robot under the influence of a motion primitive is a sequence of locations i.e., $\xi = \pose_t, \pose_{t+1}, \pose_{t+2}, \dots$ such that it satisfies the underlying dynamics in Equation~\ref{eqn:sys}.

Let $\dist{\pose}{(\vq_i,\vq_g)}$ be the distance between location $\pose_t$ and the line passing through locations $\vq_i$ and $\vq_g$.

\noindent
\textbf{\textit{$\epsilon$-tube:}}
A robot is within the $\epsilon$-tube surrounding the line passing through points $\vq_i$ and $\vq_g$, represented by $\tube{(\vq_i,\vq_g)}{\epsilon}$, if the distance between its current position and the line is bounded by $\epsilon$, i.e., 
%\begin{equation}\label{eq:tube}
$\tube{(\vq_i,\vq_g)}{\epsilon} := \{ \pose \mid \dist{\pose}{(\vq_i,\vq_g)} < \epsilon \}$.
%\end{equation}


\noindent
\textbf{\textit{Motion plan:}}
A robot moves from its current location to a destination location by executing a motion plan which is a sequence of motion primitives. For example, for a way-point based motion planner using $\goto$ motion primitive, a motion plan $\mu = \goto(\pose_1)\dots\goto(\pose_g)$ is a sequence of $\goto$'s that drives the robot from its current location to destination location $\pose_g$.  

\subsection{Overview of the Robotics Software Stack}




==> composition.tex <==
%\subsection{Correctness of an \rta System}
%\label{sec:comp}




%\textit{\textbf{Input-Output Contracts.}}
%An \rta module is an open system interacting with its environment using the input-output topics.
%When defining the semantics of an \rta module, we assumed that the environment can generate any input $v \in \val$. 
%Hence, \SC must satisfy the correctness properties \cond{P2} under any environment.
%Designing such an \SC is extremely hard and in most cases infeasible.
%In practice, a safe controller is designed under certain \textit{input assumptions}.
%Also, when an \rta module is composed with another module, the input of one module may be an output of other.
%In which case, the \rta module must provide \textit{output guarantees} that satisfy the input assumptions of the composed module.
%We would like to ensure that the output guarantee holds even when the \AC is in control.
%
%To specify simple input-output contracts, \tool allows attaching contracts to topics.
%The declaration below attaches an assumption \inlinecode{ControlRange} with the values stored at topic \inlinecode{VelocityControl}.
%
%\begin{figure}[h]
%	\centering
%	\lstinputlisting[language=modp, style=ModPCodeStyle]{./code/topics.p}
%	\vspace{-0.2cm}
%\end{figure}
%
%To capture input assumptions, the \textsc{Environment-Input} rule (Figure~\ref{fig:semantics}) is updated to allow only those values that satisfy the corresponding topic assumption.
%To provide the output guarantees, the publish semantics is updated such that a publish operation is disabled if it does not satisfy the topic assumption on which it is publishing the value.

==> implementation.tex <==

\section{\tool Tool Chain}

\label{sec:implementation}

The \tool tool-chain consists of two components: the compiler and a C runtime. 
The compiler converts the source-level syntax of a \tool program into C code. 
This code contains statically-defined C array-of-structs and functions for
the topics, nodes, and functions declarations.
The $\OEM$ that controls the output of each node is implemented as a shared-global data-structure updated by all the $\DM$s in the program.
The \tool C runtime executes the program according to the program's operational semantics by using the C representation of the nodes.
The periodic behavior of each node was implemented using OS timers for our experiments, deploying the generated code on real-time operating system is future work.

\ankush{need to add details about the testing infrastructure}



==> safecontrol.tex <==

\subsection{Obstacle Collision Avoidance}

\label{Sec:safe_MPR}
Given a high level task to visit a goal location, the motion planner computes a motion plan (sequence of motion primitives); such that the low level motion primitives can safely take the robot to the goal while avoiding collisions. 
In our case, motion plan is a sequence of $\goto$ primitives. 
The motion planner  assumes that the trajectory of a robot when executing the $\goto$ primitive always lies inside a bounded tube. 
In other words, if $\xi$ represents the trajectory of the robot when executing primitive $\goto(\pose_f)$ at location $\pose_i$ and if $\xi(t)$ represents the position of the robot in the trajectory at time $t$ then we require, $\forall t, \xi(t) \in \tube{(\pose_i,\pose_f)}{\epsilon}$ for some $\epsilon$.
We refer to $\tube{(\pose_i,\pose_f)}{\epsilon}$ as the \textit{safe-tube} for a motion-primitive $\goto(\pose_f)$ applied at position $\pose_i$.
To guarantee collision avoidance, the motion planner must then ensure that the $\epsilon$-tube surrounding the sequence of $\goto$ primitives does not collide with any obstacle.

The hard problem is computing the value of $\epsilon$ for the tube such that the $goto$ primitive provides the guarantee that any trajectory executed by it keeps the robot within the $\epsilon$-tube.
Since these motion primitives are implemented using off-the-shelf controllers or learned controllers providing such guarantees is extremely hard.

\begin{wrapfigure}{l}{0.6\columnwidth}
	\centering
	\includegraphics[scale=0.3]{figures/tube}
	\caption{Experiment to demonstrate that $\goto$ implemented using untrusted third-party controllers is unsafe}
	\label{fig:tubeexp}
\end{wrapfigure}





%\begin{wrapfigure}{l}{0.45\columnwidth}
%	\vspace{-0.75cm}
%	\centering
%	\includegraphics[scale=0.33]{figures/tube}
%	\caption{Experiment to demonstrate that $\goto$ implemented using untrusted third-party controllers is unsafe}
%	\vspace{-0.5cm}
%	\label{fig:tubeexp}
%\end{wrapfigure}

\noindent
\textbf{Experiment:} To demonstrate this problem, we experimented with a $\goto$ primitive implemented using controllers provided by the drone manufacturers. Figure~\ref{fig:tubeexp} presents the workspace consisting of a square track surround by obstacles on all sides (dashed gray area). The task for the drone was to repeatedly visit locations g1 to g4 in that order which corresponds to a motion plan {\small $\mu = \goto(g1)\goto(g2)..\goto(g4)$}. 
The blue lines represent the trajectories of the drone. 
The green region represents the safe-tube for the $\goto$ primitives.  The $\epsilon$ is chosen such that the tube does not collide with the obstacles.
%\begin{wrapfigure}{l}{0.45\columnwidth}
%	\vspace{-1cm}
%	\centering
%	\includegraphics[scale=0.23]{figures/simplextube}
%	\caption{\rta protected safe $\goto$ primitive}
%	\label{Fig:goto}
%\end{wrapfigure}
Given the complex dynamics of a drone and noisy sensors, ensuring that the drone precisely follows a fixed trajectory (ideally a straight line joining the goal locations) is extremely hard.
The untrusted low-level controllers used for implementing the $\goto$ optimizes for speed and tries to minimize the time taken to cover each segment.
Optimizing for high speed maneuvers reduces the control on the drone which leads to overshoot and trajectories that can lead to collisions (represented by the red regions). 

 

\begin{wrapfigure}{l}{0.6\columnwidth}
    	\centering
	\includegraphics[scale=0.23]{figures/simplextube}
	\caption{Regions of operation for \rta protected $\goto$ motion primitive}
	\label{Fig:goto}
\end{wrapfigure}

\noindent
\textbf{$\rta$ protected safe $\goto$:}
We next show how we construct a safe $\goto$ primitive by wrapping it inside a \rta module.
Figure~\ref{Fig:goto} presents the behavior of a safe $\goto$ represented by the \rta module $\mrta= (\mac, \msc, \period, \phisafe, \phisafer)$ where:
(1) {$\mac$} is a $\goto$ motion primitive implemented using untrusted controllers optimizing the time taken to reach $\pose_{f}$ as fast as possible.
(2) {$\msc$} is a safe controller that maintains the trajectory within the $tube(\pose_{i}, \pose_{f}, \epsilon)$. One can implement $\msc$ to be a low level controller designed for safety and that moves the drone from its current location $\pose_t$ in the switching region to a location inside $S(\phisafer, \period)$ (represented by the blue trajectory). Potential candidates for $\msc$ are bang-bang controller~\cite{bellman1956bang} or iterative linear quadratic regulators (iLQR)~\cite{DBLP:conf/icinco/LiT04}. $\msc$ must satisfy the well-formedness constraints {\footnotesize \cond{P2}} of the \rta module.
(3) $\period$ is chosen when designing $\msc$ as it must satisfy {\footnotesize \cond{P2}}.
(4) $\phisafe$ asserts that the current position $ \pose_t \in tube(\pose_{i}, \pose_{f}, \epsilon)$. The region inside the outermost tube is the safe region for the \rta module.
(5) $\phisafer$ is chosen such that $\phisafer$, $\phisafe$ and $\period$ jointly satisfy {\footnotesize \cond{P3}} and is represented by the innermost tube.
	
To compute $\ttf(\pose, \phisafe)$ accurately, we need to know the dynamics of the system. We can compute $\ttf(\pose, \phisafe)$, by exhaustively searching over all trajectories starting from $\pose$, and picking the smallest trajectory which leaves $\SR{\phisafe}{0}$. This computation is time consuming with poor scaling with dimension of $\pose$. 
In practice, we can get a conservative upper bound for $\ttf(\pose, \phisafe)$, by making the assumption that the underlying dynamics is continuous and Lipschitz bounded. 
This is a reasonable assumption to make since all physical systems are continuous, and are locally Lipschitz bounded given the control space, $\controls$, is bounded. 
%One of the techniques to compute $\ttf$ is by using the level sets of a Lyapunov function in order to quantify the Region of Attraction (ROA) of equilibrium points of a system~\cite{khalil1996noninear}.
A good approximation of the local Lipschitz bound with respect to the control is, $L_{u} = \max \frac{\partial f}{\partial u}(\pose, u)$.  Given $L_u$, we can compute the conservative $\hat{\ttf}(\pose, \phisafe) = d_{min}(\partial\SR{\phisafe}{0}, \pose)/L_{u}$, where $\partial\SR{\phisafe}{0}$ is the boundary of the safe set, and $d_{min}(\partial\SR{\phisafe}{0}, \pose)$ is minimum distance between $\pose$ and the boundary, $\partial\SR{\phisafe}{0}$ . In our drone experiment, $L_{u}$ depends on the maximum torque input, and $\partial\SR{\phisafe}{0}$ is the circumference of the safe-tube. 

In Figure~\ref{Fig:goto}, the \DM monitors the trajectory generated by $\mac$ to check if the trajectory leaves $\phisafe$ and transfers control to $\msc$ once it leaves the $S(\phisafe, 2*\period)$ tube. 
The $\msc$ is responsible for returning the drone to $S(\phisafer, \period)$, where the \DM returns control back to $\mac$ in order to maximize the usage of \AC. 
More details about the safe $\goto$ and its evaluation is provided in Section~\ref{sec:tuberesults}.

Note that $\mrta$ guarantees that all trajectories of the drone will remain inside the corresponding safe-tube irrespective of the implementation of the $\goto$ primitive i.e. $\mac$.
\textit{This is the advantage of using \rta as one can now substitute $\mac$ with any controller which maybe faulty, but the system would still remain within the safe-tube.}
The motion planner that uses the safe $\goto$ motion primitives now provide the guarantee of no obstacle collision as long as it ensures that the safe-tubes do not collide with the obstacles.









==> trustedsoftware.tex <==
\section{Runtime Assurance Protected Robotics System}

\label{sec:trustedsoftware}

In this section, we describe how the \rta module (Section~\ref{sec:simplex}) can be used to guarantee obstacle avoidance and battery safety in the presence of untrusted components.

\input{safecontrol}

\input{batterysafety}
